Treble Counterfactual VLMs: A Causal Approach to Hallucination

Vision-Language Models (VLMs) have advanced multi-modal tasks like image captioning, visual question answering, and reasoning. However, they often generate hallucinated outputs inconsistent with the visual context or prompt, limiting reliability in critical applications like autonomous driving and medical imaging. Existing studies link hallucination to statistical biases, language priors, and biased feature learning but lack a structured causal understanding. In this work, we introduce a causal perspective to analyze and mitigate hallucination in VLMs. We hypothesize that hallucination arises from unintended direct influences of either the vision or text modality, bypassing proper multi-modal fusion. To address this, we construct a causal graph for VLMs and employ counterfactual analysis to estimate the Natural Direct Effect (NDE) of vision, text, and their cross-modal interaction on the output. We systematically identify and mitigate these unintended direct effects to ensure that responses are primarily driven by genuine multi-modal fusion. Our approach consists of three steps: (1) designing structural causal graphs to distinguish correct fusion pathways from spurious modality shortcuts, (2) estimating modality-specific and cross-modal NDE using perturbed image representations, hallucinated text embeddings, and degraded visual inputs, and (3) implementing a test-time intervention module to dynamically adjust the model's dependence on each modality. Experimental results demonstrate that our method significantly reduces hallucination while preserving task performance, providing a robust and interpretable framework for improving VLM reliability. To enhance accessibility and reproducibility, our code is publicly available at https://github.com/TREE985/Treble-Counterfactual-VLMs.

==> tabs/tab4.tex <==
% \renewcommand{\arraystretch}{1.5}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
    \centering
    \vspace{5pt}
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{c c c c c c c c c c}  
        \toprule
        \textbf{NUmber of samples} & \textbf{Overall} & Attribute & Adversarial & Comparison & Counting & Relation & Environment & Holistic & Other \\
        \midrule
        Regular &2.06 &3.25 &1.83 &2.25 &2.40 &1.83  &1.92 &1.67 &1.33        \\ \cline{1-10}
        25 &2.45 & 4.17 & 1.5 & 3.67 & 1.92 & 1.83 & 2.5 & 2.0 & 2.0 \\ \cline{1-10}
        50 &2.82 &4.00 &2.17 &3.83 &2.25 &2.42 &2.83 &2.42 &2.67        \\ \cline{1-10}
        75 &2.51 &3.58&1.67&3.58&1.92&2.5&3.08&1.67&2.08   \\ \cline{1-10}
        100 &2.42 &3.58&1.67&3.08&1.75&2.08&3.08&1.58&2.5     \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{Performance of LLaVA 1.5 on MMHal-Bench with different number of samples. }
    \label{tab:Sample_performance}

\end{table*}
